Trends and Challenges in Wireless Channel Modeling for an Evolving Radio Access

With the advent of 5G, standardization and research are currently defining the next generation of the radio access. Considering the high constraints imposed by the future standards, disruptive technologies such as Massive MIMO and mmWave are being proposed. At the heart of this process are wireless channel models that now need to cover a massive increase in design parameters, a large variety of frequency bands, and heterogeneous deployments. This tutorial describes how channel models address this new level of complexity and which tools the community prepares to efficiently but accurately capture the upcoming changes in radio access design. We analyze the main drivers behind these new modeling tools, the challenges they pose, and survey the current approaches to overcome them.

==> tikzlibrarytimeline.code.tex <==
% * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
% COPYRIGHT 2014 - Claudio Fiandrino
% Released under the LaTeX Project Public License v1.3c or later
% 
% email: <claudio dot fiandrino at gmail dot com>
%
% Timeline TikZ library version 0.3a - 19/07/2014

\usetikzlibrary{backgrounds,calc}

\pgfkeys{/tikz/.cd,
  timespan/.store in=\timespan,
  timespan=Week,
  timeline width/.store in=\timelinewidth,
  timeline width=20,
  timeline height/.store in=\timelineheight,
  timeline height=1,
  timeline offset/.store in=\timelineoffset,
  timeline offset=0.15,
  initial week/.store in=\initialweek,
  initial week=1,
  end week/.store in=\endweek,
  end week=2,
  time point/.store in=\timepoint,
  time point=0.5,
  between day/.style args={#1 and #2 in #3}{% auxiliary style for days
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between week/.style args={#1 and #2 in #3}{% style for weeks
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between month/.style args={#1 and #2 in #3}{% auxiliary style for months
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between year/.style args={#1 and #2 in #3}{% auxiliary style for years
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  involvement degree/.store in=\involvdegree,
  involvement degree=2cm,
  phase color/.store in=\phasecol,
  phase color=red!50!orange,
  phase appearance/.style={
    circle,
    opacity=0.3,
    minimum size=\involvdegree,
    fill=\phasecol
  },
}
% settings to customize aspect of timeline
\newif\ifcustominterval
\pgfkeys{/tikz/timeline/.cd,
  custom interval/.is if=custominterval,
  custom interval=false,
}

% settings to deploy milestones
\pgfkeys{/tikz/milestone/.cd,
  at/.store in=\msstartpoint,
  at=phase-1.north,
  circle radius/.store in=\milestonecircleradius,
  circle radius=0.1cm,
  direction/.store in=\msdirection,
  direction=90:2cm,
  text/.store in=\mstext,
  text={},
  text options/.code={\tikzset{#1}},
}

\newcommand{\reftimespan}{\MakeLowerCase{\timespan}}

\newcommand{\timeline}[2][]{
  \pgfkeys{/tikz/timeline/.cd,#1}
  \draw[fill,opacity=0.8] (0,0) rectangle (\timelinewidth,\timelineheight);
  \shade[top color=black, bottom color=white,middle color=black!20]
    (0,0) rectangle (\timelinewidth,-\timelineoffset);
  \shade[top color=white, bottom color=black,middle color=black!20]  
    (0,\timelineheight) rectangle (\timelinewidth,\timelineheight+\timelineoffset);

  \ifcustominterval%
    \foreach \smitem [count=\xi] in {#2}  {\global\let\maxsmitem\xi}%
  \else%
    \foreach \smitem [count=\xi] in {1,...,#2}  {\global\let\maxsmitem\xi}%
  \fi%
  
  \pgfmathsetmacro\position{\timelinewidth/(\maxsmitem+1)}
  \node at (0,0.5\timelineheight)(\timespan-0){\phantom{Week 0}};
 
  \ifcustominterval%
    \foreach \x[count=\xi] in {#2}{%
      \node[text=white,text depth=0pt]at +(\xi*\position,0.5\timelineheight) (\timespan-\xi) {\timespan\ \x};%
    }%
  \else%
    \foreach \x[count=\xi] in {1,...,#2}{%
      \node[text=white, text depth=0pt]at +(\xi*\position,0.5\timelineheight) (\timespan-\xi) {\timespan\ \x};%
    }%
  \fi%  
}

\newcounter{involv}
\setcounter{involv}{0}

\newcommand{\phase}[1]{
\stepcounter{involv}
\node[phase appearance,#1] 
 (phase-\theinvolv)
 at ($(\timespan-\initialweek)!\timepoint!(\timespan-\endweek)$){};
}

\newcommand{\initialphase}[1]{
\node[phase appearance,#1,anchor=west,between week=0 and 1 in 0,] 
 (phase-\theinvolv)
 at ($(\timespan-0)!0!(\timespan-1)$){};
\setcounter{involv}{0} 
}

\newenvironment{phases}{\begin{pgfonlayer}{background}}{\end{pgfonlayer}}

\newcommand{\addmilestone}[1]{
\pgfkeys{/tikz/milestone/.cd,#1}
\draw[double,fill] (\msstartpoint) circle [radius=\milestonecircleradius];
\draw(\msstartpoint)--++(\msdirection)node[/tikz/milestone/text options]{\mstext};
}

% HISTORY
% 0.1 -> initial release
% 0.2 -> customizable timespan label
% 0.3 -> \timeline command with custom intervals
%             styles ``between x''
%             removed unnecessary call to xstring
% 0.3a -> text depth for timeline labels
